Joint Sensing and Communication over Memoryless Broadcast Channels

A memoryless state-dependent broadcast channel (BC) is considered, where the transmitter wishes to convey two private messages to two receivers while simultaneously estimating the respective states via generalized feedback. The model at hand is motivated by a joint radar and communication system where radar and data applications share the same frequency band. For physically degraded BCs with i.i.d. state sequences, we characterize the capacity-distortion tradeoff region. For general BCs, we provide inner and outer bounds on the capacitydistortion region, as well as a sufficient condition when it is equal to the product of the capacity region and the set of achievable distortion. Interestingly, the proposed synergetic design significantly outperforms a conventional approach that splits the resource either for sensing or communication.

==> Ex_bounds.tex <==

\begin{figure}[!h]
	\centering
	\vspace{-7cm}
	
	\begin{tikzpicture}[every pin/.style={fill=white},scale=.85]
	\begin{axis}[%
		xlabel={ {$D$ }},
	ylabel={ {$R_1+R_2$ }},
	xlabel style={yshift=0.2em},
	ylabel style={yshift=-1em},
%	width=.93\columnwidth,
%	width=3.028in,
%	height=2.754in,
	at={(0.611in,0.442in)},
%	scale only axis,
	xmin=0.155,
	xmax=0.185,
	ymin=0.8,
	ymax=1.6,
	xtick={0.16, 0.17, 0.18},
	axis background/.style={fill=white},
	legend pos=south east,
	legend style={legend cell align=left, align=left, draw=white!15!black}
	]
	\addplot [color=blue, line width=2.0pt]
	table[row sep=crcr]{%
		0.15625	1\\
		0.15725	1.11493262742641\\
		0.15825	1.19300663526176\\
		0.15925	1.25660468269536\\
		0.16025	1.31045924881934\\
		0.16125	1.35679912448532\\
		0.16225	1.39692059113385\\
		0.16325	1.43166498432848\\
		0.16425	1.46161569767371\\
		0.16525	1.48719457078673\\
		0.16625	1.50871456997003\\
		0.16725	1.52641087358079\\
		0.16825	1.54046022361587\\
		0.16925	1.55099339848532\\
		0.17025	1.55810337593429\\
		0.17125	1.5618506139973\\
		0.171875	1.5618506139973\\
		0.181875	1.5618506139973\\
	};
	\addlegendentry{Upper Bound from \eqref{outer}}
	
	\addplot [color=red, line width=2.0pt]
	table[row sep=crcr]{%
		0.15625	0.8125\\
		0.15725	0.96574350323521\\
		0.15825	1.06984218034902\\
		0.15925	1.15463957692714\\
		0.16025	1.22644566509246\\
		0.16125	1.28823216598042\\
		0.16225	1.34172745484513\\
		0.16325	1.38805331243798\\
		0.16425	1.42798759689828\\
		0.16525	1.46209276104897\\
		0.16625	1.49078609329337\\
		0.16725	1.51438116477439\\
		0.16825	1.53311363148783\\
		0.16925	1.5471578646471\\
		0.17025	1.55663783457905\\
		0.17125	1.5616341519964\\
		0.171875	1.5616341519964\\
		0.181875	1.5616341519964\\
	};
	\addlegendentry{Lower Bound \eqref{eq:lower_sum}}
	
	\end{axis}
	
	\begin{axis}[%
	width=7.778in,
	height=5.833in,
	at={(0in,0in)},
	scale only axis,
	xmin=0,
	xmax=1,
	ymin=0,
	ymax=2,
	axis line style={draw=none},
	ticks=none,
	axis x line*=bottom,
	axis y line*=left
	]
	\end{axis}
	\end{tikzpicture}%
	\vspace{-0.5cm}
		\caption{Upper and lower bounds  of Corollary~\ref{ex:general} on the maximum achievable sum-rate  $(R_1+R_2)$ in function of the admissible distortion $D_1=D_2$  for the state-dependent Dueck BC when $P_{S}(1)=3/4$ and $P_S(0)=1/4$.}
		\label{general_example}
		 \vspace{-.45cm}
		 
\end{figure}

